Effective model for a short Josephson junction with a phase discontinuity

We consider a short Josephson junction with a phase discontinuity $\kappa$ created, e.g., by a pair of tiny current injectors, at some point $x_0$ along the length of the junction. We derive the effective current-phase relation (CPR) for the system as a whole, i.e., reduce it to an effective point-like junction. From the effective CPR we obtain the ground state of the system and predict the dependence of its critical current on $\kappa$. We show that in a large range of $\kappa$ values the effective junction behaves as a $\varphi_0$ Josephson junction, i.e., has a unique ground state phase $\varphi_0$ within each $2\pi$ interval. For $\kappa\approx\pi$ and $x_0$ near the middle of the junction one obtains a $\varphi_0\pm\varphi$ junction, i.e., the Josephson junction with degenerate ground state phase $\varphi_0\pm\varphi$ within each $2\pi$ interval. Further, in view of possible escape experiments especially in the quantum domain, we investigate the scaling of the energy barrier and eigenfrequency close to the critical currents and predict the behavior of the escape histogram width $\sigma(\kappa)$ in the regime of the macroscopic quantum tunneling.

==> MyMc.tex <==
%%% This is 'MyMc.tex' v3.00
%%% LaTeX macros for frequently used abbreviations
%%% 13.12.2011 by Edward Goldobin <gold@uni-tuebingen.de>

\RequirePackage{xspace}

%stupid macros like \ie, \eg, \etc
\newcommand{\ie}{\textit{i.e.}\xspace}
\newcommand{\eg}{\textit{e.g.}\xspace}
\newcommand{\etal}{\textit{et al.}\xspace}
\newcommand{\cf}{\textit{cf.}\xspace}
\newcommand{\vs}{\textit{vs.}\xspace}
\newcommand{\etc}{\textit{etc.}\xspace}
\newcommand{\viz}{\textit{viz.}\xspace}
%\newcommand{\etal}{\textit{et~al.}\xspace}
\newcommand{\lhs}{l.h.s.\@\xspace}
\newcommand{\rhs}{r.h.s.\@\xspace}

\newcommand{\mum}{\ensuremath{\mathrm{\mu m}}}
\newcommand{\degree}{\ensuremath{^\circ}\xspace}

%units
\newcommand{\units}[1]{\ensuremath{\,\mathrm{#1}}}


% Convenient ratios and (partial) derivatives
%
%big \frac is called \ratio.
%usage: \ratio{a}{b}
\newcommand{\ratio}[2]{\displaystyle\frac{#1}{#2}}
%usage: \fracd{y}{x} produces fraction dy/dx.
%usage with optional argument: \fracd[2]{y}{x} produces 2nd derivative
\newcommand{\fracd}[3][]{\displaystyle\frac{d^{#1}#2}{d#3^{#1}}}
%usage: \fracp{y}{x} produces partial derivatice dy/dx.
%usage with optional argument: \fracp[2]{y}{x} produces 2nd order partial derivative
\newcommand{\fracp}[3][]{\displaystyle\frac{\partial^{#1}#2}{\partial#3^{#1}}}
%mixed derivatives are not implemented yet :-(

%Averaging macros:
%
%usage1: \av{V} - averaged V
%usage2: \av[x]{V} - V averaged with respect to x
\newcommand{\av}[2][]{\ensuremath{\left\langle#2\right\rangle_{#1}}\xspace}
%usage: \mean{u} - produced bar over the argument
\newcommand{\mean}[1]{\ensuremath{\overline{#1}}\xspace}
\newcommand{\dev}[2][]{\ensuremath{\widetilde{#2}_{#1}}\xspace}

%Freq used materials
\RequirePackage{xspace}
\newcommand{\YBCO}{YBa$_2$Cu$_3$O$_7$\xspace}
\newcommand{\LBCO}[1][x]{La$_{2-#1}$Ba$_#1$CuO$_4$\xspace}
\newcommand{\BSCCO}{Bi$_2$Sr$_2$Ca$_1$Cu$_2$O$_{8}$\xspace}
\newcommand{\NBCO}[1][x]{NdBa$_2$Cu$_3$O$_{7-#1}$\xspace}
\newcommand{\TBCO}{Tl$_2$Ba$_2$CuO$_6$\xspace}
\newcommand{\HBCO}{HgBa$_2$CuO$_6$\xspace}
\newcommand{\NCCO}{Nd$_{2-x}$Ce$_x$CuO$_4$\xspace}
\newcommand{\PCCO}{Pr$_{2-x}$Ce$_x$CuO$_4$\xspace}
\newcommand{\LCMO}[1][x]{La$_{1-#1}$Ca$_x$MnO$_3$\xspace}
\newcommand{\STO}{SrTiO$_3$\xspace}
\newcommand{\CeO}{CeO$_2$\xspace}
\newcommand{\MgB}{MgB$_2$\xspace}
\newcommand{\OrgIJJ}{$\kappa$-(BEDT-TTF)$_2$Cu(NCS)$_2$\xspace}


%technology definitions
\newcommand{\NbAlOxNb}{Nb-AlO$_x$-Nb\xspace}
\newcommand{\TechNb}{Nb-AlO$_x$-Nb\xspace}
\newcommand{\TechYBCONb}{YBCO-Nb\xspace}
%
\newcommand{\SIS}{\ensuremath{\mathrm{S|I|S}}\xspace}
\newcommand{\SNS}{\ensuremath{\mathrm{S|N|S}}\xspace}
\newcommand{\SFS}{\ensuremath{\mathrm{S|F|S}}\xspace}
\newcommand{\SIFS}{S$|$I$|$F$|$S\xspace}
\newcommand{\SfiS}{S$|$FI$|$S\xspace}
%\newcommand{\SJS}{\ensuremath{\mathrm{S-FI-S}}\xspace}

%%
%% Freq used math symbols
%%

%Elliptic fns
\newcommand{\am}{\mathop{\mathrm{am}}\nolimits}
\newcommand{\dn}{\mathop{\mathrm{dn}}\nolimits}
\newcommand{\sn}{\mathop{\mathrm{sn}}\nolimits}
\newcommand{\cn}{\mathop{\mathrm{cn}}\nolimits}
\newcommand{\gd}{\mathop{\mathrm{gd}}\nolimits}
\newcommand{\E} {\mathop{\mathrm{E}}\nolimits}
\newcommand{\F} {\mathop{\mathrm{F}}\nolimits}
\newcommand{\K} {\mathop{\mathrm{K}}\nolimits}
\newcommand{\J}[1][] {\mathop{\mathrm{J_{#1}}}\nolimits}
\newcommand{\Ai} {\mathop{\mathrm{Ai}}\nolimits}
\newcommand{\Bi} {\mathop{\mathrm{Bi}}\nolimits}

%Other fns
%\newcommand{\const}{\mathop{const}\nolimits}
\newcommand{\atanh}{\mathop{\mathrm{atanh}}\nolimits}
\newcommand{\acot}{\mathop{\mathrm{acot}}\nolimits}
\newcommand{\sech}{\mathop{\mathrm{sech}}\nolimits}
\newcommand{\sgn}{\mathop{\mathrm{sgn}}\nolimits}
\newcommand{\floor}{\mathop{\mathrm{floor}}\nolimits}
\newcommand{\ceil}{\mathop{\mathrm{ceil}}\nolimits}
\newcommand{\const}{\mathop{\mathrm{const}}\nolimits}
\renewcommand{\Re}{\mathop{\mathrm{Re}}\nolimits}
\renewcommand{\Im}{\mathop{\mathrm{Im}}\nolimits}
%\angle(sin,cos) returns the angle if sin and cos are known
\newcommand{\ang}{\mathop{\mathrm{ArcSinCos}}\nolimits}
%\newcommand{\O} {\mathop{\mathrm{O}}\nolimits} %of the order of

%\newcommand{\Det}{\mathop{\mathrm{det}}\nolimits}
%\newcommand{\Tr}{\mathop{\mathrm{Tr}}\nolimits}

\newcommand{\qstate}[1]{\ensuremath{\left\lvert\state{#1}\right\rangle}}
\newcommand{\rot}{\mathop\mathrm{\mathbf{rot}}\nolimits}
\newcommand{\grad}{\mathop\mathbf{{\rm grad}}\nolimits}
%\newcommand{\div}{\mathop{{\rm div}}\nolimits}


%just shortcuts
%\newcommand{\HS}{\ensuremath{{\cal H}}}
\newcommand{\Heavyside}{\mathop{\mathrm{H}}\nolimits}
\newcommand{\G}{\ensuremath{{\cal G}}}
\newcommand{\Dx}{\ensuremath{{\Delta x}}}
\newcommand{\dx}{\ensuremath{{\delta x}}}
\newcommand{\Dw}{\ensuremath{{\Delta w}}}
\newcommand{\D}[1]{\ensuremath{{\Delta #1}}}
%\newcommand{\d}[1]{\ensuremath{{\delta #1}}}

%\iffalse%{
\RequirePackage{amssymb}

% macros for showing/hiding corrections

%\RequirePackage[normalem]{ulem}

%\newcommand{\new}[1]{\textcolor{blue}{#1}}
%\newcommand{\del}[1]{\textcolor{red}{\sout{#1}}}
%\newcommand{\chg}[1]{\textcolor{magenta}{#1}}
\RequirePackage{ifthen}
\newboolean{ShowCorrections}
\setboolean{ShowCorrections}{true}%<-- set here show/notshow corrections

%%%Reduction/Corrections macros
\ifthenelse{\boolean{ShowCorrections}}{%
\usepackage[normalem]{ulem}%
\newcommand{\new}[1]{\textcolor[rgb]{0,0,1}{#1}}%
\newcommand{\old}[1]{\textcolor[rgb]{1,0,0}{\sout{#1}}}%
}{%
\newcommand{\new}[1]{#1}%
\newcommand{\old}[1]{}%
}


%%
%% Not allowed stuff
%%

%state command which may not translate correctly
\newcommand{\stat}[1]{\state{#1}}

%%tth:\def\relax{}
%%tth:\def\message#1{}

%\tracingmacros=2
%%%%%%%%%%

\def\state#1{\ensuremath{\stt#1.}}
\def\stt#1{%
\if#1.
\let\next=\relax
\else
  \if#1u
    \upharpoonleft%\uparrow
  \else\if#1d
    \downharpoonleft%\downarrow
  \else\if#1U
    \upharpoonright%\Uparrow
  \else\if#1D
    \downharpoonright%\Downarrow
  \else\if#1F
    \Uparrow
  \else\if#1A
    \Downarrow
  \else\if#1s
    \uparrow
  \else\if#1a
    \downarrow
  \else\if#1r
    \rightarrow
  \else\if#1l
    \leftarrow
  \else\if#1R
    \Rightarrow
  \else\if#1L
    \Leftarrow
  \else\if#1>
    \longrightarrow
  \else\if#1<
    \longleftarrow
  \else\if#1
  \relax
  \else
  ?\message{Unknown symbol #1 in the argument of macro state}
  \fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi
\let\next=\stt
\fi
\next
}

%usage: \hstruct{Nb|Al|Nb}
%at the moment cannot accept math or lower indices. :-(
\def\hstruct#1{%
\let\accu=\relax%
\hstruc#1.%
\accu
}
\def\hstruc#1{%
\if#1.%end?
\let\next=\relax
\else
  \if#1|%
    \let\accu=\accu$|$%
%  \else\if#1
%    \relax
  \else
    \let\accu=\accu #1%\message{Unknown symbol #1 in the argument of macro \hstruc}
  \fi%\fi
  \let\next=\hstruc
\fi
\next
}


\newcounter{CurrTimeHH}\newcounter{CurrTimeMM}
\newcommand{\CurrTime}{%
  \setcounter{CurrTimeHH}{\time/60}%
  \setcounter{CurrTimeMM}{\time - \value{CurrTimeHH}*60}%
  \ifthenelse{\value{CurrTimeHH}<10}{0}{}\theCurrTimeHH:%
  \ifthenelse{\value{CurrTimeMM}<10}{0}{}\theCurrTimeMM%
}



